Delivering Inflated Explanations

In the quest for Explainable Artificial Intelligence (XAI) one of the questions that frequently arises given a decision made by an AI system is, ``why was the decision made in this way?'' Formal approaches to explainability build a formal model of the AI system and use this to reason about the properties of the system. Given a set of feature values for an instance to be explained, and a resulting decision, a formal abductive explanation is a set of features, such that if they take the given value will always lead to the same decision. This explanation is useful, it shows that only some features were used in making the final decision. But it is narrow, it only shows that if the selected features take their given values the decision is unchanged. It's possible that some features may change values and still lead to the same decision. In this paper we formally define inflated explanations which is a set of features, and for each feature of set of values (always including the value of the instance being explained), such that the decision will remain unchanged. Inflated explanations are more informative than abductive explanations since e.g they allow us to see if the exact value of a feature is important, or it could be any nearby value. Overall they allow us to better understand the role of each feature in the decision. We show that we can compute inflated explanations for not that much greater cost than abductive explanations, and that we can extend duality results for abductive explanations also to inflated explanations.

==> ack.tex <==
\ack
%
This work was supported by the AI Interdisciplinary Institute ANITI,
funded by the French program ``Investing for the Future -- PIA3''
under Grant agreement no.\ ANR-19-PI3A-0004,
%
by the H2020-ICT38 project COALA ``Cognitive Assisted agile
manufacturing for a Labor force supported by trustworthy Artificial
intelligence'',
%
by the National Research Foundation, Prime Minister’s Office,
Singapore under its Campus for Research Excellence and Technological
Enterprise (CREATE) programme,
%
and by the Australian Government through the Australian Research Council Industrial Transformation Training Centre in Optimisation Technologies, Integrated Methodologies, and Applications (OPTIMA), Project ID IC200100009.%
%This work received comments and suggestions from several colleagues,
%including
%N.\ Asher, M.\ Cooper, %E.\ Hebrard,
%A.\ Ignatiev,
%J.\ Planes, A.\ Morgado,
%%C.\ Menc\'{\i}a,
%and N.\ Narodytska.
%%, R.\ Passos and J.\ Planes.
%%

